Improving Metrology with Quantum Scrambling

Quantum scrambling describes the spreading of local information into many degrees of freedom in quantum systems. This provides the conceptual connection among diverse phenomena ranging from thermalizing quantum dynamics to models of black holes. Here we experimentally probe the exponential scrambling of a multi-particle system near a bistable point in phase space and utilize it for entanglement-enhanced metrology. We use a time-reversal protocol to observe a simultaneous exponential growth of both the metrological gain and the out-of-time-order correlator, thereby experimentally verifying the relation between quantum metrology and quantum information scrambling. Our experiments demonstrate that fast-scrambling dynamics capable of exponentially fast entanglement generation are useful for practical metrology, resulting in 6.8(4) dB gain beyond the Standard Quantum Limit.

==> method.tex <==
\newpage
\section*{Methods}
% \def\thesection{}
% \section{TODO}
% We should write the technical appendices / methods first: these will not change no matter how we sell the story. 

% Here are the list of necessary technical parts:
% \begin{itemize}
%     \item loading \textcolor{red}{DONE}
%     \item different sequences
%     \item two-color squeezing and characterization [ZL]
%     \item amplification protocol
%     \item measurements \textcolor{red}{DONE}
%     \item tomography [ZL]
%     \item Holstein-primakoff and equivalence to TAT [ZL] 
% \end{itemize}

\section*{Loading}
We load $^{171}$Yb atoms from a Yb dispenser into a two-color mirror magneto-optical trap (MOT) on the singlet ${^1S_0}{\rightarrow} {^1P_1}$ and triplet ${^1S_0}{\rightarrow} {^3P_1}$ transitions.
%
In this stage, the atoms are cooled down to $\approx 1$~mK, close to the Doppler limit imposed by the strong dipole transition (i.e., the singlet transition).
%
Subsequently, the are loaded into a second-stage green MOT on the narrower linewidth triplet transition that allows for a compressed ($\approx 100~\mathrm{\mu m}$) and colder atomic cloud ($\approx 20 \mathrm{\mu K}$).
%
By moving the zero magnetic field point, the atomic cloud is transported into the cavity TEM$_{00}$ mode at a distance of $\Delta z \approx 50 \mathrm{~\mu m}$ from the cavity waist~\cite{Kawasaki2020}. 
%

The trap is formed, through the cavity, by a standing-wave `magic-wavelength' light with $\lambda_t\approx759$~nm.
%
At the atom location, the trap depth is $U_0 = k_B~120\times\mathrm{\mu K}$.
%
Since the trapping light is always on, simply turning off the green MOT transfers the atoms into the optical lattice.
%
However, before turning of the green MOT light, we reduce the light intensity and simultaneously increase the red detuning of the frequency, this last step allows us to compensate for the differential Stark shift induced by the trapping light which on the triplet state ${}^3P1$ is $25\%$ larger than on the ground state.   

In this way, an ensemble of atoms is prepared at a distance of $\approx 50$~$\mu$m from the cavity mode waist.
%

\section*{Characterizing single-atom cooperativity}

We characterize the single-atom cooperativity $\eta$ by measuring the spin projection noise via the cavity as a function of the collective cooperativity $N\eta$, where $N$ is the total number of atoms coupled to the cavity.
%
For a coherent spin state (CSS) prepared at the equator of the generalized Bloch sphere, the measured variance of the difference is %= \frac{\eta}{2} \aver{\hat{N}_\uparrow- \hat{N}_\downarrow}$} is 
\begin{equation}
\mathrm{var}(\eta S_z)=(N\eta)\frac{\eta}{4}.
\end{equation}
%
The latter contribution is obtained through the variance of the difference between two measurements after a single CSS preparation.

%%%% -- Fig Single Atom Cooperativity
\begin{figure}[!ht]
    \centering
    \includegraphics[width=.85\columnwidth]{figure/etaMeasurment.pdf}
    \caption{Measured variance of $\eta S_z$ as a function of the average collective cooperative $N\eta$. When we are spin-projection limited, we have a linear relation with slope $\eta/4$.}
    \label{fig:singleatomCooperativity}
\end{figure}

%%% -------------------

Plotting the variance of $\eta S_z$ as a function of the collective cooperativity results, in the absence of classical sources of noise, in a linear graph with slope $\eta/4$ (see fig.~\ref{fig:singleatomCooperativity}).
%
We subtract the measurement resolution contribution to the variance and we obtain single-atom cooperativity $\eta = 8.8\pm0.3$ by fitting the data to a linear model. 

When a quadratic fitting term is included to account for possible technical noise, we recover the same cooperativity $\eta=8.2 \pm 1.1$ within error bars. Moreover, the coefficient of the second order terms agrees with 0.


 


\section*{Hamiltonian}
The Hamiltonian is implemented by adding the two parts of Hamiltonian, OAT Hamiltonian and transverse Rabi field together
\begin{align}
    \hat{H}=\hat{H}_\mathrm{OAT}+\hat{H}_\mathrm{trans}=\chi\hat{S}_z^2+\Omega{\bf n}\cdot\hat{\bf S},
\end{align}
where $\hat{\bf S}$ is a vector operator of the collective spin with the total length $S$, while its $x, y, z$-components $\hat{S}_{x,y,z}=\frac{1}{2} \sum_{j} \hat{\sigma}_{x,y,z}^j$. We can control $\chi, \Omega$ as described below, and the ${\bf n}$ by controlling the RF field's phase and frequency. In this work, we don't use any $\hat{S}_z$ rotation, and thus phase is enough to control ${\bf n}$ in the x-y plane. 
\subsection{Magnetic Rabi frequency}
We characterize our maximum magnetic field strength $\Omega_\mathrm{max}$ by a Rabi sequence, i.e., after the optical pumping, we continuously apply $\Omega\hat{S}_x$ Hamiltonian for time $t$ and measure the $\langle \hat{S}_z\rangle$. We typically get maximally $\Omega_\mathrm{max}=2\pi\times220$Hz. We can control the strength relative to the maximal value precisely through the analog channel of a National Instrument card. 


\subsection{Squeezing strength}
% $N\chi$ and $\Omega$ characterization. 
The squeezing strength is characterized by the anti-squeezing under pure OAT Hamiltonian, which scales as $\mathrm{var}(\hat{S}_y)=1+\dot{F}t+(N\chi t)^2$. By fitting we obtain both the measurement rate $\dot{F}$ and the squeezing strength $N\chi$, whose ratio agrees with the theoretical calculation using parameters in Table~\ref{tab:my_label}.


\section*{Two-color Interaction}

The atoms are trapped by an optical lattice formed by the cavity mode at 759nm, and the cavity light which generates the OAT Hamiltonian is at 556nm. Thus, atoms trapped at different lattice site may experience different atom-light interaction strength (cooperativity). The collective behavior can still be captured by an effective atom number and effective cooperativity~\cite{Hu2015}; however, to obtain the ideal Hamiltonian with no detuning, we need to cancel the first order phase shift term $\hat{H}_0\propto\hat{S}_z$~\cite{Li2022}. We cannot use a detuning in RF field to cancel that because each atom experiences different local light field and therefore different detuning should be applied. 

To overcome this, we simultaneously send two frequencies of light into the cavity, both generating the same squeezing sign but but with opposite light-shift term; the linear $S_z$ term of the Hamiltonian is then cancelled by carefully tuning the amplitude of the two sidebands . The idea is similar to our previous setups~\cite{Braverman2019,Colombo2022}; the difference is this time we send the light simultaneously. In order to do that we generate RF signals with two individually controlled frequencies and intensities from two voltage-controlled oscillators, both with voltage controlled attenuator. The two signals are added via an RF splitter, and then amplified and and used to drive the EOM. In this case, the full Hamiltonian~\cite[Eq.~(14)]{Li2022}'s electric field is the sum of two components with different frequencies, which individually generates the OAT and first order phase shift. 
%

The Hamiltonian also contains an interference term which oscillates at the beat frequency. For the practical experiment configuration this beating frequency is always much higher than all other related energy scale and therefore can be neglected. The final parameters we choose with $N\eta=2000$ and $\eta\sim 9$ are given in Table.~\ref{tab:my_label}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{c|c|c}
         & Frequency 1 [MHz] & Frequency 2 [MHz] \\\hline
        Squeezing ($\chi>0$) & $8.93$ & $-2.19$ \\\hline
        Un-Squeezing ($\chi<0$) & $-8.9$ & $2.25$ \\\hline
    \end{tabular}
    \caption{Parameters of two-color interaction}
    \label{tab:my_label}
\end{table}

% Specifically, for the squeezing part we used 


\section*{State measurement}
%
% The value of \red{$\aver{\hat{S}_z}$} is obtained from the difference \red{$\hat{S}_z{=}(\hat{N}_\uparrow{-}\hat{N}_\downarrow){/}2$} of the populations \red{$\hat{N}_\uparrow$} and \red{$\hat{N}_\downarrow$} of the states $\ket{\uparrow}$ and $\ket{\downarrow}$, respectively.
The single measurement outcome of $\hat{S}_z$ is obtained from the difference ${S}_z{=}({N}_\uparrow{-}{N}_\downarrow){/}2$ of the populations $N_\uparrow$ and $N_\downarrow$ of the states $\ket{\uparrow}$ and $\ket{\downarrow}$, respectively. 
We first measure the $N_\uparrow$ through the vacuum Rabi splitting of the cavity mode $2g{\approx}\sqrt{N_\uparrow\eta\kappa\Gamma}$ when the empty cavity is resonant with the transition $\ket{\uparrow}\rightarrow\ket{e}=\ket{^3P_1, m_F=+3/2}$~\cite{Braverman2019}. 
Here $\kappa{=}2\pi{\times}530(10)~$kHz is the cavity linewidth and $\Gamma{=}2\pi{\times}184(1)~$kHz the linewidth of the atomic transition. The Rabi splitting is measured by scanning the laser frequency and detecting the cavity transmission as a function of the frequency. To measure $N_\downarrow$ we swap the population between the $\ket{\uparrow}$ and $\ket{\downarrow}$ states through the application of an rf $\pi$-pulse and repeating the measurement procedure described above. The sum $N_\uparrow + N_\downarrow$ gives the total atom number $N$ in one experimental shot.  

%
The resolution of a single measurement, normalized to the SQL, is given by $\sigma_d^2= \frac{1}{S_0}\mathrm{var}(S_{z1}-S_{z2})$ where $S_{z1}$ and $S_{z2}$ are two state measurements performed after a single CSS preparation. We obtain $\sigma_d^2{=}0.15\pm0.02$ and it remains constant within the whole range of atom numbers used in this experiment. 
%
For the experiments requiring a measurement of any other projection of the spin vector, we apply a dedicated rf-pulse that maps the desired projection onto the $\hat{S}_z$ one.

\section*{Quantum state tomography and Fidelity OTOC}

We implement a quantum state tomography on the symmetric sub Hilbert space of collective spin states~\cite{Schmied2011}. For each quantum state, we measure the spin projection along 41 different directions on the Bloch sphere with in total more than 1200 measurements, and reconstructed on a $N=200$ ($S=N/2=100$)'s 101-dimensional Hilbert space. Each measurement result is translated to a projection operator and fed into the algorithm to reconstruct a density matrix $\rho$. 

% As in~\cite{Lewis2019}, we can measure the fidelity OTOC (FOTOC) by tomographically reconstruct the density matrix of the time-reversed perturbed state $\rho'(0)$ and calculate the overlap with a CSS along $x$-direction.  
% \[\begin{aligned}
% \mathcal{F}_{G}(t, \delta \phi) & \equiv\left\langle\hat{W}_{G}^{\dagger}(t) \hat{\rho}(0) \hat{W}_{G}(t) \hat{\rho}(0)\right\rangle \\
% &=\operatorname{Tr}\left(\rho^{\prime}(0) \rho(0)\right)%\\
% % &=\left|\left\langle\psi_{0}\left|e^{i \hat{H} t} e^{i \delta \phi \hat{G}} e^{-i \hat{H} t}\right| \psi_{0}\right\rangle\right|^{2} \\
% % & \approx 1-\delta \phi^{2} \operatorname{var}[\hat{G}(t)]
% \end{aligned}\]
% where here $\rho_0$ represents the CSS along $x$-direction, $\hat{W}_G(0)=e^{-i\hat{G}\delta\phi}$, and $\hat{G} = \hat{S}_\alpha$ is the sensitivity rotation direction. 

% The expression of FOTOC under the unitary evolution condition can be further expressed as
% \[\begin{aligned}
% \mathcal{F}_{G}(t, \delta \phi) &=\left|\left\langle\psi_{0}\left|e^{i \hat{H} t} e^{i \delta \phi \hat{G}} e^{-i \hat{H} t}\right| \psi_{0}\right\rangle\right|^{2} \\
% & \approx 1-\delta \phi^{2} \operatorname{var}[\hat{G}(t)],
% \end{aligned}\]
% and we make a quadratic fit over $\delta\phi$ to infer the scrambling coefficient (also known as Fisher information or metrological gain) of our system. 

